Analysis of the Compaction Behavior of Textile Reinforcements in Low-Resolution In-Situ CT Scans via Machine-Learning and Descriptor-Based Methods

A detailed understanding of material structure across multiple scales is essential for predictive modeling of textile-reinforced composites. Nesting -- characterized by the interlocking of adjacent fabric layers through local interpenetration and misalignment of yarns -- plays a critical role in defining mechanical properties such as stiffness, permeability, and damage tolerance. This study presents a framework to quantify nesting behavior in dry textile reinforcements under compaction using low-resolution computed tomography (CT). In-situ compaction experiments were conducted on various stacking configurations, with CT scans acquired at 20.22 $\mu$m per voxel resolution. A tailored 3D{-}UNet enabled semantic segmentation of matrix, weft, and fill phases across compaction stages corresponding to fiber volume contents of 50--60 %. The model achieved a minimum mean Intersection-over-Union of 0.822 and an $F1$ score of 0.902. Spatial structure was subsequently analyzed using the two-point correlation function $S_2$, allowing for probabilistic extraction of average layer thickness and nesting degree. The results show strong agreement with micrograph-based validation. This methodology provides a robust approach for extracting key geometrical features from industrially relevant CT data and establishes a foundation for reverse modeling and descriptor-based structural analysis of composite preforms.

==> figures/fig_D_s2_160.tex <==
\begin{tikzpicture}[trim axis left, trim axis right]
    \begin{axis}[
        colormap={plasma}{ % Define Plasma colormap manually
            rgb=(0.050383,0.029803,0.527975)
            rgb=(0.213753,0.000000,0.800000)
            rgb=(0.497000,0.000000,0.831373)
            rgb=(0.735683,0.000000,0.745189)
            rgb=(0.901961,0.294118,0.294118)
            rgb=(0.986000,0.730000,0.184000)
            rgb=(0.940015,0.975158,0.131326)
        },
        axis on top,
        enlargelimits=false,
        % colorbar, % Optional: Colorbar won’t affect the PNG itself
        xlabel={$x$ \tikzArrow}, ylabel={$y$ \tikzArrow},
        width=.5\columnwidth,
        height=.5\columnwidth,
    ]
        \addplot graphics [xmin=0, xmax=220, ymin=0, ymax=150] {figures/fig_D_s2_160/s2_phase0_xy.png};
    \end{axis}
\end{tikzpicture}

==> figures/fig_F-delta_phi.tex <==
\begin{tikzpicture}[
                trim axis left,
                trim axis right,
                clip=True
                ]
    \begin{axis}[
        % xmin=0, xmax=4500,
        % ymin=0, ymax=800,
        width=0.4*\textwidth, height=0.4*\textwidth,
        % xtick={0,500,1000,1500,2000,2500,3000,3500,4000,4500}, 
        % xticklabels={\num{0},\num{.5},\num{1},\num{1.5},\num{2},
        % \num{2.5},\num{3},\num{3.5},$[\si{\second}]$,\num{4.5}},
        % ytick={0,200,400,600,800}, 
        % yticklabels={\num{0},\num{200},\num{400},[\si{\newton}],\num{800}},
        xlabel={$t$ \tikzArrow}, 
        ylabel={$F$ \tikzArrow},
        xmajorgrids,
        ymajorgrids,
        clip=false,
        legend pos=south east,
        legend cell align=left,
        legend style={cells={align=left}, font=\footnotesize},
        % domain=-50:100.0,
    ]

   

    
    \addplot[thick,
        draw,
        color=plasma7,
    ] table[x=force_N, y=delta_mm,col sep=comma] {figures/fig_t-F_delta_acq/285_10_layer_machine_data_red.csv};
    \addlegendentry{$F_z$}






    
    \end{axis}





    
\end{tikzpicture}
